Differentiable Safe Controller Design through Control Barrier Functions

Learning-based controllers, such as neural network (NN) controllers, can show high empirical performance but lack formal safety guarantees. To address this issue, control barrier functions (CBFs) have been applied as a safety filter to monitor and modify the outputs of learning-based controllers in order to guarantee the safety of the closed-loop system. However, such modification can be myopic with unpredictable long-term effects. In this work, we propose a safe-by-construction NN controller which employs differentiable CBF-based safety layers, and investigate the performance of safe-by-construction NN controllers in learning-based control. Specifically, two formulations of controllers are compared: one is projection-based and the other relies on our proposed set-theoretic parameterization. Both methods demonstrate improved closed-loop performance over using CBF as a separate safety filter in numerical experiments.

==> old_simulation_draft.tex <==
\section{Simulations}
\subsection{Benchmark comparisons}
To demonstrate the effectiveness and advantages of our proposed method, we compare it with two of the most common approaches.
\begin{enumerate}
    \item Neural network (NN);
    \item Projection neural network (Projection NN).
\end{enumerate}
\subsection{2D Double Integrator for Obstacle Avoidance}
Consider a linear 2D double integrator:
\begin{align}
    \Dot{\bold{x}} = A\bold{x} + B\bold{u}
\end{align}
where we set the sampling time $\Delta t$ as $0.2s$.
\begin{align}
h(\bold{x})=1-(x_1+2.5)^2-(x_2+2.5)^2
\end{align}

\subsection{Inverted Pendulum Stabilization}
We then consider the application of controlling simulated inverted pendulum, which has mass $m$, length $l$, the inertia $I$, the angle $\theta$, and is actuated by control input $u$.
The gravitational constant is $g$.
The inverted pendulum is modeled by using the following first order ODE system:
\begin{align}\label{model:pendulumcont}
    \begin{bmatrix}
\Dot{x_1}\\
\Dot{x_2}
\end{bmatrix} = 
\begin{bmatrix}
0 & 1\\
-a_0 & -a_1
\end{bmatrix}
\begin{bmatrix}
x_1\\
x_2
\end{bmatrix} 
+ 
\begin{bmatrix}
0\\
b_0
\end{bmatrix}u
\end{align}
with $a_0=-\frac{mgl}{I+ml^2}, a_1=\frac{b}{I+ml^2}, b_0=\frac{ml}{I+ml^2}$, where $x_1 = \theta, x_2 = \Dot{\theta}$. 
Safety specification is the angular velocity (i.e., $\dot{\theta}$) is no less than $-0.5$, which means that the safe set is 
\begin{align}
\mathcal{C}=\{\bold{x}: x_2+0.5\ge 0\},   
\end{align}
where the control barrier function could be defined as $h(\bold{x})=x_2-0.5$.

Discretize the continuous-time system (\ref{model:pendulumcont}) and the time step is $0.2s$.
We first collect dataset from MPC-based pendulum control, and then train the neural network using supervised learning framework.
The results are shown in Figures.
It can be shown that the pure NN method is not safe, and project NN and gauge NN methods could preserve safety.
The running time of these three methods are similar in this case, since the dimension of the control input is only 1 and thus the LP/QP take little time.

\begin{figure}
    \centering
    \includegraphics[width=5cm]{figures/nn.png}
    \caption{NN}
    \label{fig:gaugennInverted}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=5cm]{figures/projectnn.png}
    \caption{Project NN}
    \label{fig:gaugennInverted}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=5cm]{figures/gaugenn.png}
    \caption{Gauge NN}
    \label{fig:gaugennInverted}
\end{figure}

\section{Discussion}
\begin{itemize}
    \item How to find the explicit feasible point of the safe set? If we can find it, we can avoid real time optimization and thus improve computational efficiency further;
    \item We need to validate the computational efficiency on a more complex example further;
    \item How to construct a generalized gauge map, which could directly map the learning component's output to the safe set without shifting the safe set. Or we can also try to learn such a generalized gauge map.
    \item Consider extending the framework to multi-agents system.
    \item Consider optimizing policy by reinforcement learning.
\end{itemize}


